Correlation between Gyral Size, Brain Size, and Head Impact Risk across Mammalian Species

A study on primates has established that gyral size is largely independent of overall brain size. Building on this, and other research suggesting that brain gyrification may mitigate the effects of head impacts, our study aims to explore potential correlations between gyral size and the risk of head impact across a diverse range of mammalian species. Our findings corroborate the idea that gyral sizes are largely independent of brain sizes, especially among species with larger brains, thus extending this observation beyond primates. Preliminary evidence also suggests a correlation between an animal's gyral size and its lifestyle, particularly in terms of head-impact risk. For instance, goats, known for their headbutting behaviors, exhibit smaller gyral sizes. In contrast, species such as manatees and dugongs, which typically face lower risks of head impact, have lissencephalic brains. Additionally, we explore mechanisms that may explain how narrower gyral sizes could offer protective advantages against head impact. Finally, we discuss a possible trade-off associated with gyrencephaly.

==> brain_samples/brains_smooth_brain_size_merged.tex <==
\begin{tabular}{c|lllc}
\hline
\textbf{Hemisphere size (cm)} & \textbf{Common name} & \textbf{Species name} & \textbf{Order} & \textbf{Brain size (cm)} \\
\hline
\hline
0.3--0.4 & Lesser horseshoe bat\cite[\#62-127]{www.brainmuseum.org}& {\it Rhinolophus hipposideros }& Chiroptera & 0.68 \\
\hline
0.5--0.6 & House mouse\cite[\#59-387]{www.brainmuseum.org}& {\it Mus musculus }& Rodentia & 1.0 \\
 & Merriam's kangaroo rat\cite[\#70-238]{www.brainmuseum.org}& {\it Dipodomys merriami }& Rodentia & 1.1 \\
\hline
0.6--0.7 & Common shrew\cite[\#64-25]{www.brainmuseum.org}& {\it Sorex araneus }& Eulipotyphla & 1.2 \\
 & North American deermouse\cite[\#59-390]{www.brainmuseum.org}& {\it Peromyscus maniculatus gracilis }& Rodentia & 1.3 \\
 & Eastern mole\cite[\#59-267]{www.brainmuseum.org}& {\it Scalopus aquaticus }& Eulipotyphla & 1.4 \\
\hline
0.7--0.8 & Mongolian gerbil\cite[\#60-352]{www.brainmuseum.org}& {\it Meriones unguiculatus }& Rodentia & 1.5 \\
 & Sugar glider\cite[\#64-20]{www.brainmuseum.org}& {\it Petaurus breviceps }& Diprotodontia & 1.5 \\
 & Degu\cite[\#66-40]{www.brainmuseum.org}& {\it Octodon degus }& Rodentia & 1.6 \\
 & Brown rat (Norway rat)\cite[\#63-463]{www.brainmuseum.org}& {\it Rattus norvegicus }& Rodentia & 1.6 \\
\hline
0.8--0.9 & Edible dormouse\cite[\#61-614]{www.brainmuseum.org}& {\it Glis glis }& Rodentia & 1.6 \\
 & Southern flying squirrel\cite[\#60-92]{www.brainmuseum.org}& {\it Glaucomys volans }& Rodentia & 1.7 \\
\hline
0.9--1.0 & Thirteen-lined ground squirrel\cite[\#67-132]{www.brainmuseum.org}& {\it Ictidomys tridecemlineatus }& Rodentia & 1.8 \\
 & Northern treeshrew\cite[\#62-279]{www.brainmuseum.org}& {\it Tupaia glis }& Scandentia & 1.8 \\
 & Greater glider\cite[\#64-37]{www.brainmuseum.org}& {\it Petauroides volans }& Diprotodontia & 2.0 \\
 & Tailless tenrec\cite[\#70-89]{www.brainmuseum.org}& {\it Tenrec ecaudatus }& Afrosoricida & 2.0 \\
 & Common ringtail possum\cite[\#64-19]{www.brainmuseum.org}& {\it Pseudocheirus peregrinus }& Diprotodontia & 2.0 \\
 & Squirrel glider\cite[\#64-28]{www.brainmuseum.org}& {\it Petaurus norfolcensis }& Diprotodontia & 2.0 \\
\hline
1.0--1.1 & Muskrat\cite[\#63-112]{www.brainmuseum.org}& {\it Ondatra zibethicus }& Rodentia & 2.1 \\
 & Bennett's chinchilla rat\cite[\#66-39]{www.brainmuseum.org}& {\it Abrocoma bennettii }& Rodentia & 2.1 \\
\hline
1.1--1.2 & Pygmy anteater\cite[Fig.~6]{10.1111/ahe.12501}& {\it Cyclopes didactylus }& Pilosa & 2.3 \\
 & Philippine tarsier\cite[\#61-193]{www.brainmuseum.org}& {\it Carlito syrichta }& Primates & 2.3 \\
\hline
1.2--1.3 & Long-tailed chinchilla\cite[\#65-103]{www.brainmuseum.org}& {\it Chinchilla lanigera }& Rodentia & 2.4 \\
 & Nine-banded armadillo\cite[Fig.~5]{10.1111/ahe.12501}& {\it Dasypus novemcinctus }& Cingulata & 2.4 \\
\hline
1.3--1.4 & Mountain beaver\cite[\#64-103]{www.brainmuseum.org}& {\it Aplodontia rufa }& Rodentia & 2.6 \\
 & Eastern gray squirrel\cite[\#60-144]{www.brainmuseum.org}& {\it Sciurus carolinensis }& Rodentia & 2.6 \\
 & Common brushtail possum\cite[\#64-29]{www.brainmuseum.org}& {\it Trichosurus vulpecula }& Diprotodontia & 2.8 \\
\hline
1.4--1.5 & European (domestic) rabbit\cite[\#73-211]{www.brainmuseum.org}& {\it Oryctolagus cuniculus }& Lagomorpha & 2.9 \\
 & Woodchuck (groundhog)\cite[\#61-770]{www.brainmuseum.org}& {\it Marmota monax }& Rodentia & 3.0 \\
\hline\end{tabular}

==> brain_samples/brains_with_sulci_hint_merged.tex <==
\begin{tabular}{c|lllc}
\hline
\textbf{Drawn size (cm)} & \textbf{Common name} & \textbf{Species name} & \textbf{Order} & \textbf{Brain size (cm)} \\
\hline
\hline
0.5--0.6 & Senegal bushbaby\cite[\#61-686]{www.brainmuseum.org}& {\it Galago senegalensis }& Primates & 1.9 \\
 & Long-nosed potoroo\cite[\#65-55]{www.brainmuseum.org}& {\it Potorous tridactylus }& Diprotodontia & 2.4 \\
\hline
0.6--0.7 & Guinea pig\cite[Fig.~2]{10.1159/000123814}& {\it Cavia porcellus }& Rodentia & 2.0 \\
 & Guinea pig\cite[\#60-1]{www.brainmuseum.org}& {\it Cavia porcellus }& Rodentia & 2.0 \\
\hline
0.7--0.8 & Common marmoset\cite[\#54-64]{www.brainmuseum.org}& {\it Callithrix jacchus }& Primates & 2.5 \\
 & Tammar wallaby\cite[\#64-33]{www.brainmuseum.org}& {\it Macropus eugenii }& Diprotodontia & 2.9 \\
\hline
0.8--0.9 & Indian flying fox\cite[\#61-617]{www.brainmuseum.org}& {\it Pteropus giganteus }& Chiroptera & 2.5 \\
\hline
1.6--1.7 & Dugong\cite[Fig.~3]{10.1111/j.1439-0469.1985.tb00577.x}& {\it Dugong dugon }& Sirenia & 6.6 \\
 & Florida manatee\cite[\#85-32]{www.brainmuseum.org}& {\it Trichechus manatus latirostris }& Sirenia & 8.3 \\
\hline
1.9--2.0 & Florida manatee\cite[Fig.~20]{10.1017/S1464793106007019}& {\it Trichechus manatus latirostris }& Sirenia & 8.4 \\
\hline\end{tabular}

==> brain_samples/combined_GS1_GS2_brains_merged_1.tex <==
\begin{tabular}{c|lllcc}
\hline
\textbf{Gyral size (cm)} & \textbf{Common name} & \textbf{Species name} & \textbf{Order} & \textbf{Brain size (cm)} & \textbf{Method} \\
\hline
\hline
0.3--0.4 & Ermine\cite[\#63-10]{www.brainmuseum.org}& {\it Mustela erminea }& Carnivora & 1.7& 1 \\
\hline
0.4--0.5 & Collared anteater\cite[Fig.~6]{10.1111/ahe.12501}& {\it Tamandua tetradactyla }& Pilosa & 1.8& 1 \\
 & Philippine flying lemur\cite[\#63-271]{www.brainmuseum.org}& {\it Cynocephalus volans }& Dermoptera & 2.4& 1 \\
 & European polecat (ferret)\cite[\#58-323]{www.brainmuseum.org}& {\it Mustela putorius }& Carnivora & 2.5& 1 \\
 & Brown greater galago\cite[\#62-172]{www.brainmuseum.org}& {\it Otolemur crassicaudatus }& Primates & 2.6& 1 \\
 & Giant anteater\cite[Fig.~6]{10.1111/ahe.12501}& {\it Myrmecophaga tridactyla }& Pilosa & 2.6& 1 \\
 & Striped skunk\cite[\#63-113]{www.brainmuseum.org}& {\it Mephitis mephitis }& Carnivora & 2.6& 1 \\
 & American mink\cite[\#58-324]{www.brainmuseum.org}& {\it Neovison vison }& Carnivora & 2.7& 1 \\
 & Yellow mongoose\cite[\#61-766]{www.brainmuseum.org}& {\it Cynictis penicillata }& Carnivora & 2.7& 1 \\
 & Rock hyrax\cite[\#62-635]{www.brainmuseum.org}& {\it Procavia capensis }& Hyracoidea & 3.0& 1 \\
 & Potto\cite[\#62-441]{www.brainmuseum.org}& {\it Perodicticus potto }& Primates & 3.0& 1 \\
 & Cat\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Felis catus }& Carnivora & 3.4& 1 \\
 & White-nosed coati\cite[\#58-360]{www.brainmuseum.org}& {\it Nasua narica }& Carnivora & 3.7& 1 \\
 & Raccoon\cite[\#57-88]{www.brainmuseum.org}& {\it Procyon lotor }& Carnivora & 4.3& 1 \\
 & White-lipped peccary\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Tayassu pecari  }& Artiodactyla & 4.5& 2 \\
 & Goat\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Capra aegagrus hircus }& Artiodactyla & 5.2& 1 \\
 & Greater kudu\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Tragelaphus strepsiceros }& Artiodactyla & 6.8& 1 \\
\hline
0.5--0.6 & Slow loris\cite[\#62-181]{www.brainmuseum.org}& {\it Nycticebus coucang }& Primates & 2.9& 1 \\
 & Common wombat\cite[\#64-11]{www.brainmuseum.org}& {\it Vombatus ursinus }& Diprotodontia & 3.1& 1 \\
 & Brown-throated sloth\cite[Fig.~4]{10.1111/ahe.12501}& {\it Bradypus variegatus }& Pilosa & 3.2& 1 \\
 & Ringtail cat\cite[\#62-106]{www.brainmuseum.org}& {\it Bassariscus astutus }& Carnivora & 3.4& 1 \\
 & Linnaeus's two-toed sloth\cite[\#61-98]{www.brainmuseum.org}& {\it Choloepus didactylus }& Pilosa & 3.5& 1 \\
 & Red panda\cite[\#60-121]{www.brainmuseum.org}& {\it Ailurus fulgens }& Carnivora & 3.8& 1 \\
 & Linnaeus's two-toed sloth\cite[Fig.~1]{10.1111/ahe.12501}& {\it Choloepus didactylus }& Pilosa & 3.9& 1 \\
 & Cat\cite[\#60-330]{www.brainmuseum.org}& {\it Felis catus }& Carnivora & 4.0& 1 \\
 & Tayra\cite[\#69-56]{www.brainmuseum.org}& {\it Eira barbara }& Carnivora & 4.1& 2 \\
 & Collared peccary\cite[\#63-445]{www.brainmuseum.org}& {\it Pecari tajacu }& Artiodactyla & 4.2& 2 \\
 & Crab-eating raccoon\cite[\#68-312]{www.brainmuseum.org}& {\it Procyon cancrivorus }& Carnivora & 4.6& 1 \\
 & American badger\cite[\#63-127]{www.brainmuseum.org}& {\it Taxidea taxus }& Carnivora & 4.9& 1 \\
 & Domestic pig\cite[\#61-361]{www.brainmuseum.org}& {\it Sus scrofa domesticus }& Artiodactyla & 5.3& 2 \\
 & Domestic goat\cite[\#59-55]{www.brainmuseum.org}& {\it Capra hircus domestica }& Artiodactyla & 5.5& 2 \\
 & Domestic sheep\cite[\#61-693]{www.brainmuseum.org}& {\it Ovis aries }& Artiodactyla & 5.8& 2 \\
 & Mouflon\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Ovis orientalis }& Artiodactyla & 6.3& 1 \\
 & White-tailed deer\cite[\#67-81]{www.brainmuseum.org}& {\it Odocoileus virginianus }& Artiodactyla & 6.9& 2 \\
 & Ganges river dolphin\cite[Fig.~19]{10.1159/000454797}& {\it Platanista gangetica }& Cetacea & 7.4& 2 \\
 & California sea lion\cite[Fig.~18]{10.1017/S1464793106007019}& {\it Zalophus californianus }& Carnivora & 7.9& 1 \\
 & Northern fur seal\cite[\#61-511]{www.brainmuseum.org}& {\it Callorhinus ursinus }& Carnivora & 8.8& 1 \\
 & Black rhinoceros \cite[Fig.~1]{10.3389/fnana.2017.00074}& {\it Diceros bicornis  }& Perissodactyla & 11& 2 \\
 & Bottlenose dolphin\cite[Fig.~2]{10.1159/000063731}& {\it Tursiops truncatus }& Cetacea & 11& 1 \\
 & Beluga whale\cite[Fig.~19]{10.1159/000454797}& {\it Delphinapterus leucas }& Cetacea & 18& 2 \\
 & Beluga whale\cite[Fig.~1]{10.1002/ar.10183}& {\it Delphinapterus leucas }& Cetacea & 19& 1 \\
\hline\end{tabular}

==> brain_samples/combined_GS1_GS2_brains_merged_2.tex <==
\begin{tabular}{c|lllcc}
\hline
\textbf{Gyral size (cm)} & \textbf{Common name} & \textbf{Species name} & \textbf{Order} & \textbf{Brain size (cm)} & \textbf{Method} \\
\hline
\hline
0.6--0.7 & Red-bellied titi monkey\cite[\#70-355]{www.brainmuseum.org}& {\it Callicebus moloch }& Primates & 3.1& 1 \\
 & Collared anteater\cite[\#61-93]{www.brainmuseum.org}& {\it Tamandua tetradactyla }& Pilosa & 3.4& 1 \\
 & Fennec fox\cite[\#63-388]{www.brainmuseum.org}& {\it Vulpes zerda }& Carnivora & 3.5& 1 \\
 & Grison\cite[\#69-11]{www.brainmuseum.org}& {\it Galictis vittata }& Carnivora & 3.6& 1 \\
 & Ring-tailed lemur\cite[\#62-442]{www.brainmuseum.org}& {\it Lemur catta }& Primates & 3.8& 1 \\
 & Short-beaked echidna\cite[\#64-232]{www.brainmuseum.org}& {\it Tachyglossus aculeatus }& Monotremata & 3.9& 2 \\
 & Domestic Dog (Beagle)\cite[\#59-326]{www.brainmuseum.org}& {\it Canis lupus familiaris }& Carnivora & 5.1& 2 \\
 & Capybara\cite[Fig.~2]{10.1159/000123814}& {\it Hydrochoerus hydrochaeris }& Rodentia & 5.2& 1 \\
 & Geoffroy's spider monkey\cite[\#63-18]{www.brainmuseum.org}& {\it Ateles geoffroyi }& Primates & 5.3& 1 \\
 & Cougar (puma)\cite[\#60-206]{www.brainmuseum.org}& {\it Puma concolor }& Carnivora & 5.6& 1 \\
 & Domestic pig\cite[Fig.~7]{10.1002/cne.25461}& {\it Sus scrofa domesticus  }& Artiodactyla & 5.9& 1 \\
 & Cheetah\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Acinonyx jubatus }& Carnivora & 6.3& 1 \\
 & African wild dog\cite[Fig.~3]{10.1002/cne.24999}& {\it Lycaon pictus }& Carnivora & 6.4& 1 \\
 & Wild boar\cite[Fig.~7]{10.1002/cne.25461}& {\it Sus scrofa }& Artiodactyla & 6.6& 1 \\
 & Llama\cite[\#65-139]{www.brainmuseum.org}& {\it Lama glama }& Artiodactyla & 6.7& 2 \\
 & Harbor seal\cite[\#61-515]{www.brainmuseum.org}& {\it Phoca vitulina }& Carnivora & 9.0& 1 \\
 & California sea lion\cite[Fig.~1]{10.1002/ar.20937}& {\it Zalophus californianus }& Carnivora & 9.5& 1 \\
 & Cattle\cite[Fig.~1]{10.1371/journal.pone.0154580}& {\it Bos taurus }& Artiodactyla & 9.9& 1 \\
 & Bactrian camel\cite[Fig.~2]{Camelus}& {\it Camelus bactrianus }& Artiodactyla & 10& 1 \\
 & Dromedary camel\cite[\#60-227]{www.brainmuseum.org}& {\it Camelus dromedarius }& Artiodactyla & 11& 2 \\
 & California sea lion\cite[Fig.~7]{10.1002/cne.23984}& {\it Zalophus californianus }& Carnivora & 11& 2 \\
 & African elephant\cite[\#85-33]{www.brainmuseum.org}& {\it Loxodonta africana }& Proboscidea & 18& 2 \\
 & Killer whale\cite[Fig.~1]{10.1017/S1464793106007019}& {\it Orcinus orca }& Cetacea & 22& 2 \\
 & Killer whale\cite[Fig.~19]{10.1159/000454797}& {\it Orcinus orca }& Cetacea & 26& 1 \\
\hline
0.7--0.8 & Olingo\cite[\#62-113]{www.brainmuseum.org}& {\it Bassaricyon gabbii }& Carnivora & 3.1& 1 \\
 & Mongoose lemur\cite[\#64-69]{www.brainmuseum.org}& {\it Eulemur mongoz }& Primates & 3.5& 1 \\
 & Kinkajou\cite[\#58-365]{www.brainmuseum.org}& {\it Potos flavus }& Carnivora & 3.6& 1 \\
 & Domestic Dog (Basenji)\cite[\#66-165]{www.brainmuseum.org}& {\it Canis lupus familiaris }& Carnivora & 4.5& 2 \\
 & Red fox\cite[\#63-392]{www.brainmuseum.org}& {\it Vulpes vulpes }& Carnivora & 4.7& 1 \\
 & Coyote\cite[\#62-301]{www.brainmuseum.org}& {\it Canis latrans }& Carnivora & 5.2& 2 \\
 & Lar gibbon\cite[\#60-142]{www.brainmuseum.org}& {\it Hylobates lar }& Primates & 5.2& 1 \\
 & Gray wolf\cite[\#71-26]{www.brainmuseum.org}& {\it Canis lupus }& Carnivora & 5.3& 2 \\
 & Capybara\cite[\#62-621]{www.brainmuseum.org}& {\it Hydrochoerus hydrochaeris }& Rodentia & 5.5& 2 \\
 & Leopard\cite[\#63-261]{www.brainmuseum.org}& {\it Panthera pardus }& Carnivora & 6.3& 2 \\
 & Hamadryas baboon\cite[Fig.~1]{10.1002/cne.903110109}& {\it Papio hamadryas }& Primates & 8.4& 1 \\
 & Common chimpanzee\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Pan troglodytes }& Primates & 8.5& 2 \\
 & Burchell's zebra\cite[\#61-820]{www.brainmuseum.org}& {\it Equus quagga burchellii }& Perissodactyla & 8.9& 2 \\
 & Pygmy hippopotamus\cite[Fig.~1]{10.1002/ar.22875}& {\it Hexaprotodon liberiensis }& Artiodactyla & 9.0& 1 \\
 & Pygmy sperm whale\cite[Fig.~2]{10.1002/ar.23991}& {\it Kogia breviceps }& Cetacea & 9.3& 1 \\
 & Hippopotamus\cite[Fig.~2]{10.1002/cne.23930}& {\it Hippopotamus amphibius }& Artiodactyla & 9.5& 2 \\
 & California sea lion\cite[\#62-294]{www.brainmuseum.org}& {\it Zalophus californianus }& Carnivora & 10& 2 \\
 & White rhinoceros\cite[Fig.~2]{10.3389/fnana.2017.00074}& {\it Ceratotherium simum }& Perissodactyla & 10& 2 \\
 & Steller sea lion\cite[\#61-513]{www.brainmuseum.org}& {\it Eumetopias jubatus }& Carnivora & 10& 2 \\
 & Horse\cite[Fig.~1]{10.1159/000356527}& {\it Equus caballus }& Perissodactyla & 12& 1 \\
 & Giraffe\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Giraffa camelopardalis }& Artiodactyla & 12& 2 \\
 & Northern elephant seal\cite[Fig.~9]{10.1002/cne.24188}& {\it Mirounga angustirostris }& Carnivora & 12& 1 \\
\hline\end{tabular}

==> brain_samples/combined_GS1_GS2_brains_merged_3.tex <==
\begin{tabular}{c|lllcc}
\hline
\textbf{Gyral size (cm)} & \textbf{Common name} & \textbf{Species name} & \textbf{Order} & \textbf{Brain size (cm)} & \textbf{Method} \\
\hline
\hline
0.8--0.9 & Rhesus monkey\cite[\#69-307]{www.brainmuseum.org}& {\it Macaca mulatta }& Primates & 5.1& 1 \\
 & Northern plains gray langur\cite[\#62-179]{www.brainmuseum.org}& {\it Semnopithecus entellus }& Primates & 6.4& 1 \\
 & Spotted hyena\cite[\#64-352]{www.brainmuseum.org}& {\it Crocuta crocuta }& Carnivora & 6.5& 2 \\
 & Mandrill\cite[\#63-310]{www.brainmuseum.org}& {\it Mandrillus sphinx }& Primates & 6.7& 1 \\
 & Mandrill\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Mandrillus sphinx  }& Primates & 6.8& 1 \\
 & American black bear\cite[\#71-256]{www.brainmuseum.org}& {\it Ursus americanus }& Carnivora & 6.8& 2 \\
 & Guinea baboon\cite[\#64-12]{www.brainmuseum.org}& {\it Papio papio }& Primates & 7.2& 1 \\
 & Lion\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Panthera leo }& Carnivora & 7.9& 1 \\
 & Zebu\cite[\#64-322]{www.brainmuseum.org}& {\it Bos taurus indicus }& Artiodactyla & 9.6& 2 \\
 & Common chimpanzee\cite[Fig.~1]{10.1002/ar.a.20256}& {\it Pan troglodytes }& Primates & 11& 1 \\
 & Giraffe\cite[Fig.~1]{10.1002/ar.23593}& {\it Giraffa camelopardalis }& Artiodactyla & 14& 1 \\
 & Sperm whale\cite[Fig.~2]{10.1002/ar.23991}& {\it Physeter macrocephalus }& Cetacea & 18& 1 \\
 & African elephant\cite[Fig.~1]{10.1002/cne.23817}& {\it Loxodonta africana }& Proboscidea & 21& 1 \\
 & Minke whale\cite[Fig.~19]{10.1159/000454797}& {\it Balaenoptera acutorostrata }& Cetacea & 22& 1 \\
 & Fin whale\cite[Fig.~1]{10.1002/ar.20407}& {\it Balaenoptera physalus }& Cetacea & 23& 2 \\
 & Minke whale\cite[Fig.~4]{10.1016/S0165-02700200182-6}& {\it Balaenoptera acutorostrata }& Cetacea & 25& 1 \\
\hline
0.9--1.0 & Giant anteater\cite[\#67-29]{www.brainmuseum.org}& {\it Myrmecophaga tridactyla }& Pilosa & 5.1& 1 \\
 & Tonkean macaque\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Macaca tonkeana  }& Primates & 6.8& 2 \\
 & Lion\cite[\#62-79]{www.brainmuseum.org}& {\it Panthera leo }& Carnivora & 7.6& 1 \\
 & Yellow baboon\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Papio cynocephalus  }& Primates & 8.0& 2 \\
 & Giant panda\cite[Fig.~3]{10.1002/cne.900840102}& {\it Ailuropoda melanoleuca }& Carnivora & 8.3& 1 \\
 & Western gorilla\cite[\#81-127]{www.brainmuseum.org}& {\it Gorilla gorilla }& Primates & 8.5& 1 \\
 & Common chimpanzee\cite[\#63-307]{www.brainmuseum.org}& {\it Pan troglodytes }& Primates & 8.6& 1 \\
 & Western lowland gorilla\cite[Fig.~1]{10.1002/ajp.20048}& {\it Gorilla gorilla gorilla }& Primates & 9.7& 1 \\
 & Polar bear\cite[\#62-250]{www.brainmuseum.org}& {\it Ursus maritimus }& Carnivora & 9.8& 1 \\
 & Hippopotamus\cite[Fig.~2]{10.1002/ar.23991}& {\it Hippopotamus amphibius }& Artiodactyla & 10& 1 \\
 & Bornean orangutan\cite[Fig.~2]{10.1002/ar.a.20256}& {\it Pongo pygmaeus  }& Primates & 11& 1 \\
 & California sea lion\cite[Fig.~10]{10.1002/cne.24188}& {\it Zalophus californianus }& Carnivora & 12& 1 \\
 & Human\cite[\#69-314]{www.brainmuseum.org}& {\it Homo sapiens }& Primates & 15& 2 \\
 & Humpback whale\cite[Fig.~1]{10.1007/s00429-014-0860-3}& {\it Megaptera novaeangliae }& Cetacea & 18& 1 \\
\hline
1.0--1.1 & Mountain gorilla\cite[Fig.~1]{10.1002/ajp.20048}& {\it Gorilla beringei beringei }& Primates & 9.6& 2 \\
 & Brown bear\cite[Fig.~1]{10.3389/fnana.2019.00079}& {\it Ursus arctos }& Carnivora & 9.8& 1 \\
 & Human\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Homo sapiens }& Primates & 13& 2 \\
 & Common chimpanzee\cite[Fig.~1]{10.3389/fnana.2020.00055}& {\it Pan troglodytes }& Primates & 14& 1 \\
\hline
1.1--1.2 & Brown bear\cite[Fig.~7]{10.3389/fnana.2011.00029}& {\it Ursus arctos  }& Carnivora & 11& 1 \\
 & Humpback whale\cite[Fig.~2]{10.1002/ar.20407}& {\it Megaptera novaeangliae }& Cetacea & 26& 1 \\
\hline
1.2--1.3 & Asian elephant\cite[Fig.~5]{10.1016/j.brainresbull.2006.03.016}& {\it Elephas maximus }& Proboscidea & 23& 1 \\
 & Asian elephant\cite[Fig.~7]{10.1016/j.brainresbull.2006.03.016}& {\it Elephas maximus }& Proboscidea & 24& 1 \\
\hline
1.4--1.5 & Bowhead whale\cite[Fig.~1]{10.1002/ar.23991}& {\it Balaena mysticetus }& Cetacea & 25& 1 \\
\hline\end{tabular}

==> brain_samples/dimple_merged.tex <==
\begin{tabular}{lllc}
\hline
 \textbf{Common name} & \textbf{Species name} & \textbf{Order} & \textbf{Brain size (cm)} \\
\hline
West European hedgehog\cite[\#61-559]{www.brainmuseum.org}& {\it Erinaceus europaeus }& Eulipotyphla & 2.0 \\
Snowshoe hare\cite[\#64-120]{www.brainmuseum.org}& {\it Lepus americanus }& Lagomorpha & 2.9 \\
North American porcupine\cite[\#62-541]{www.brainmuseum.org}& {\it Erethizon dorsatum }& Rodentia & 3.8 \\
North American beaver\cite[\#63-168]{www.brainmuseum.org}& {\it Castor canadensis }& Rodentia & 3.9 \\
North American beaver\cite[Fig.~4]{10.1159/000123818}& {\it Castor canadensis }& Rodentia & 4.8 \\
\hline\end{tabular}

==> brain_samples/irregular_merged.tex <==
\begin{tabular}{lllc}
\hline
 \textbf{Common name} & \textbf{Species name} & \textbf{Order} & \textbf{Brain size (cm)} \\
\hline
Nine-banded armadillo\cite[\#60-465]{www.brainmuseum.org}& {\it Dasypus novemcinctus }& Cingulata & 2.9 \\
Three-striped night monkey\cite[\#69-255]{www.brainmuseum.org}& {\it Aotus trivirgatus }& Primates & 2.9 \\
Tasmanian pademelon\cite[\#65-59]{www.brainmuseum.org}& {\it Thylogale billardierii }& Diprotodontia & 3.3 \\
Common squirrel monkey\cite[\#61-672]{www.brainmuseum.org}& {\it Saimiri sciureus }& Primates & 3.4 \\
Mantled howler\cite[\#68-409]{www.brainmuseum.org}& {\it Alouatta palliata }& Primates & 4.3 \\
Western grey kangaroo\cite[\#62-127]{www.brainmuseum.org}& {\it Macropus fuliginosus }& Diprotodontia & 4.7 \\
Greater spot-nosed monkey\cite[\#63-490]{www.brainmuseum.org}& {\it Cercopithecus nictitans }& Primates & 5.4 \\
Collared mangabey\cite[\#63-489]{www.brainmuseum.org}& {\it Cercocebus torquatus }& Primates & 6.6 \\
\hline\end{tabular}
